Belief Propagation Reloaded: Learning BP-Layers for Labeling Problems

It has been proposed by many researchers that combining deep neural networks with graphical models can create more efficient and better regularized composite models. The main difficulties in implementing this in practice are associated with a discrepancy in suitable learning objectives as well as with the necessity of approximations for the inference. In this work we take one of the simplest inference methods, a truncated max-product Belief Propagation, and add what is necessary to make it a proper component of a deep learning model: We connect it to learning formulations with losses on marginals and compute the backprop operation. This BP-Layer can be used as the final or an intermediate block in convolutional neural networks (CNNs), allowing us to design a hierarchical model composing BP inference and CNNs at different scale levels. The model is applicable to a range of dense prediction problems, is well-trainable and provides parameter-efficient and robust solutions in stereo, optical flow and semantic segmentation.

==> 04_bp_layer.tex <==
\section{\bpl}
\label{sec:bpLayer}
In \cref{sec:lbp} we have reviewed the general multi-class classification problem and how it can be approximately solved with Loopy Belief Propagation (LBP). 
However, the LBP algorithm cannot be used for learning yet.
We are going to show how we can use the LBP algorithm as a general building block for dense prediction tasks in the following.
We call the learnable BP algorithm {\em \bpl}.

\subsection{From LBP algorithm to \bpl}


Let the nodes $i$ in one row be enumerated from $1, \dots N$. 
If we insert $j = i+1$ in \cref{eq:messageUpdates}, we get the message updates for the left-right sweep.
The task is now to compute the derivative of the beliefs $b$ \wrt the data-term $g$ for every node in the graph for every label, \ie
\begin{equation}
    \frac{\partial b_i(s)}{\partial g_j(t)} = \frac{\partial b_i(s)}{\partial m_i(u)} \sum_D \left(\frac{\partial m_{i}(u)}{\partial m_j^D(v)} \frac{\partial m_j^D(v)}{\partial g_j(t)}\right),
\end{equation}
where $D={L,R,U,D}$ is the set of direction. 
The difficult part is the message-to-message derivative in the sum, because here we need to traverse the graph backwards to compute the gradients.
\todo{is this sum correct(?)}

\begin{equation} \label{eq:b_d}
b_d := \frac{ \partial b_{ij}(s)}{\partial m_{ij}^d(p)} = 1
\end{equation}
 
\begin{equation} \label{eq:m_U}
m_U := \prod_{i'= i}^{k + 2} \frac{\partial m_{i' j}^U(p_{i'})}{\partial m_{i'-1 j}^U(q_{i'})} = \prod_{i'= i}^{k + 2} \llbracket s_{i' j}^{*^U} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:m_D}
m_D := \prod_{i'= i}^{k - 2} \frac{\partial m_{i' j}^D(p_{i'})}{\partial m_{i'+1 j}^D(q_{i'})} = \prod_{i'= i}^{k - 2} \llbracket s_{i' j}^{*^D} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:m_L}
m_L := \prod_{j'= j}^{l + 2} \frac{\partial m_{i j'}^L(p_{i'})}{\partial m_{i j'-1}^L(q_{i'})} = \prod_{j'= j}^{l + 2} \llbracket s_{i j'}^{*^L} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:m_R}
m_R := \prod_{j'= j}^{l - 2} \frac{\partial m_{i j'}^R(p_{i'})}{\partial m_{i j'+1}^R(q_{i'})} = \prod_{j'= j}^{l - 2} \llbracket s_{i j'}^{*^R} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:g_U}
g_U := \frac{\partial m_{k+1 l}^U(q)}{\partial g_{k l}(t)} = \llbracket s_{k+1 l}^{*^U} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:g_D}
g_D := \frac{\partial m_{k-1 l}^D(q)}{\partial g_{k l}(t)} = \llbracket s_{k-1 l}^{*^D} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:g_L}
g_L := \frac{\partial m_{k l+1}^L(q)}{\partial g_{k l}(t)} = \llbracket s_{k l+1}^{*^L} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:g_R}
g_R := \frac{\partial m_{k l-1}^R(q)}{\partial g_{k l}(t)} = \llbracket s_{k l-1}^{*^R} = s \rrbracket
\end{equation}

\begin{equation} \label{eq:m_DR}
m_{DR} := \frac{\partial m_{k-1 j}^D(q)}{\partial m_{k j}^R(v)} = \llbracket s_{k-1,j}^{*^D} =  s\rrbracket
\end{equation}

\begin{equation} \label{eq:m_UL}
m_{UL} := \frac{\partial m_{k+1 j}^U(q)}{\partial m_{k j}^L(v)}= \llbracket s_{k+1,j}^{*^U} =  s\rrbracket
\end{equation}

We demonstrate the gradient computation on a

\input{04_tikz_bp_minimal.tex}

We want to compute the derivative of the beliefs $b$ \wrt to the unary costs $g$. Thus we are interested in computing
\begin{equation}
    \frac{\partial b}{\partial g_{kl}(t)} = \sum_{i, j}^{M,N} \frac{\partial b_{ij}(s)}{\partial g_{kl}(t)},
    \label{eq:gradG} 
\end{equation}
where $i$ and $j$ are source and $k$ and $l$ are target positions on the 2D pixel grid, $s$ is the source label and $t$ is the target label.
The terms of the sum are dependent on the source and target position and are given by
\begin{equation}
    \frac{\partial b_{ij}(s)}{\partial g_{kl}(t)}
    =
    \begin{cases}
        b_U \delta_U g_U & \text{if } i > k, j = l \\
        b_D \delta_D g_D & \text{if } i < k, j = l \\
        b_L \delta_L g_L & \text{if } i = k, j > l \\
        b_R \delta_R g_R & \text{if } i = k, j < l \\
        b_D \delta_D m_{DR} \delta_R g_R & \text{if } i < k, j < l \\
        b_U \delta_U m_{UL} \delta_L g_L & \text{if } i > k, j > l \\
        \frac{\partial b_{ij}}{\partial g_{kl}} & \text{if } i = k, j = l \\
    \end{cases}
\end{equation}
The sub-scripts indicate the direction, \ie L(eft), R(ight), U(p), D(own), the delta-functions enable or disable propagation along the chain and double sub-scripts indicate cross-connections.
\begin{equation}
    \delta_U =
    \begin{cases}
    1 & \text{if } i < k + 2 \\
    m_U & \text{else} 
    \end{cases}
    \label{eq:deltaU}
\end{equation}
\begin{equation}
    \delta_D =
    \begin{cases}
    1 & \text{if } i > k - 2 \\
    m_D & \text{else} 
    \end{cases}
    \label{eq:deltaD}
\end{equation}
\begin{equation}
    \delta_L =
    \begin{cases}
    1 & \text{if } j < l + 2 \\
    m_L & \text{else} 
    \end{cases}
    \label{eq:deltaL}
\end{equation}
\begin{equation}
    \delta_R =
    \begin{cases}
    1 & \text{if } j > l - 2 \\
    m_R & \text{else} 
    \end{cases}
    \label{eq:deltaR}
\end{equation}


Since we have a $\min$ in the forward pass, only those labels being on the optimal path will get a gradient. 
This can be seen in the indicator functions in \cref{eq:m_U,eq:m_D,eq:m_L,eq:m_R,eq:g_U,eq:g_D,eq:g_L,eq:g_R}.


\begin{algorithm}[t]
  \KwIn{$\dv{B_{ij}}$: incoming gradient, $amin_{ij}$: argmin from forward path}
  \KwOut{$\dv{g_{ij}}$, gradient for unary costs}
   {\bf Init:} $\dv{g_{ij}} := \dv{B_{ij}},~A_{d}=0~\forall D, G_{dij}=0:D \in \{ U, D \}$, initialize unary gradient with $b_d := \frac{ \partial b_{ij}(s)}{\partial m_{ij}^d(p)} \cdot \dv{B_{ij}} = \dv{B_{ij}}$, init accumulator variable $A$ with zero, init U,D gradient save variable $G_{dij}$ with zero
   
    \For{$d \in \{ U, D \}$}
    {
       \eIf{$d = U$}
       { 
       \For{$i=N-2 \dots 0$}
       { 
         $s^* = amin_{i+1j}$\; 
         \For{$k=0 \dots K$}
         {
           $z = B_{i+1j}(k) + A_{d}(k)$\;
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + z$\;
           $a_{d}(s^*(k)) = a_{d}(s^*(k)) + z$\;
         }
         \For{$k=0 \dots K$}
         {
           $A_{d}(k) = a_{d}(k)$\;
         }
         $G_{dij} = \dv{g_{ij}}$\;
       }
       }
       {
       \For{$i=1 \dots N$}
       {
          $s^* = amin_{i-1j}$\; 
         \For{$k=0 \dots K$}
         {
           $z = B_{i-1j}(k) + A_{d}(k)$\;
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + z$\;
           $a_{d}(s^*(k)) = a_{d}(s^*(k)) + z$\;
         }
         
         \For{$k=0 \dots K$}
         {
           $A_{d}(k) = a_{d}(k)$\;
         }
          $G_{dij} = \dv{g_{ij}}$\;
       }
     
       }
    }
    
    \Return $\dv{g_{ij}}$
\caption{Min-sum unary gradient implementation pseudo-code part 1}
\end{algorithm}

\begin{algorithm}[t]
  \KwIn{$\dv{B_{ij}}$: incoming gradient, $amin_{ij}$: argmin from forward path, $G_{dij}$: saved gradients from part 1}
  \KwOut{$\dv{g_{ij}}$, gradient for unary costs}
   {\bf Init:} $\dv{g_{ij}} := \dv{B_{ij}},~A_{d}=0~\forall D$, initialize unary gradient with $b_d := \frac{ \partial b_{ij}(s)}{\partial m_{ij}^d(p)} \cdot \dv{B_{ij}} = \dv{B_{ij}}$, init accumulator variable $A$ with zero
   

    \For{$d \in \{ R, L \}$}
    {
      \eIf{$d = L$}
       { 
       \For{$j=N-2 \dots 0$}
       { 
         $s^* = amin_{ij+1}$\; 
         \For{$k=0 \dots K$}
         {
           $z = B_{ij+1}(k) + A_{d}(k)$\;
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + z$\;
           $a_{d}(s^*(k)) = a_{d}(s^*(k)) + z$\;
           
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + + G_{Uij+1}(k) + A_{U}(k)$\;
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + G_{Dij+1}(k) + A_{D}(k)$\;
           
           $a_{U}(s^*(k)) = a_{U}(s^*(k)) + G_{Uij+1}(k) + A_{U}(k)$\;
           $a_{D}(s^*(k)) = a_{U}(s^*(k)) + G_{Dij+1}(k) + A_{D}(k)$\;
         }
         \For{$k=0 \dots K$}
         {
           $A_{d}(k) = a_{d}(k)$\;
         }
       }
      
       }
       {
       \For{$j=1 \dots N$}
       {
          $s^* = amin_{ij-1}$\; 
         \For{$k=0 \dots K$}
         {
           $z = B_{ij-1}(k) + A_{d}(k)$\;
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + z$\;
           $a_{d}(s^*(k)) = a_{d}(s^*(k)) + z$\;
           
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + + G_{Uij-}(k) + A_{U}(k)$\;
           $\dv{g_{ij}}(s^*(k)) = \dv{g_{ij}}(s^*(k)) + G_{Dij-1}(k) + A_{D}(k)$\;
           
           $a_{U}(s^*(k)) = a_{U}(s^*(k)) + G_{Uij-1}(k) + A_{U}(k)$\;
           $a_{D}(s^*(k)) = a_{U}(s^*(k)) + G_{Dij-1}(k) + A_{D}(k)$\;
         }
         \For{$k=0 \dots K$}
         {
           $A_{d}(k) = a_{d}(k)$\;
         }
       }
     
       }
    
    }
    \Return $\dv{g_{ij}}$
\caption{Min-sum unary gradient implementation pseudo-code part 2}
\end{algorithm}


\begin{itemize}
    \item Standard: Unrolling the iterates
    \item Show that one interate is sufficient
    \item Compute gradients 
    \item Show correctness of gradients
\end{itemize}

\subsection{Properties of the \bpl}
\begin{itemize}
    \item Compute FLOPS for Min-Sum/Sum-Prod and compare with 3D convs
    \item Make example where the long-range propagation is beneficial (e.g. large untextured region)
    
\end{itemize}
